pfd-parallel, a Singular/GPI-Space package for massively parallel multivariate partial fractioning

Multivariate partial fractioning is a powerful tool for simplifying rational function coefficients in scattering amplitude computations. Since current research problems lead to large sets of complicated rational functions, performance of the partial fractioning as well as size of the obtained expressions are a prime concern. We develop a large scale parallel framework for multivariate partial fractioning, which implements and combines an improved version of Leinartas' algorithm and the {\sc MultivariateApart} algorithm. Our approach relies only on open source software. It combines parallelism over the different rational function coefficients with parallelism for individual expressions. The implementation is based on the \textsc{Singular}/\textsc{GPI-Space framework} for massively parallel computer algebra, which formulates parallel algorithms in terms of Petri nets. The modular nature of this approach allows for easy incorporation of future algorithmic developments into our package. We demonstrate the performance of our framework by simplifying expressions arising from current multiloop scattering amplitude problems.

==> IBP_table.tex <==



==> compression_ratio.tex <==
\subsection{Reduction coefficients simplification achieved by PFD program}\label{sec:compression}

  Our PFD implementation using the Singular/GPI-Space framework can simplify the $19.6$ GB of the original reduction coefficients to $186$ MB
  within $72$ hours of parallel computation, utilizing $350$ cores and relying only on parallelization over the different IBP coefficients. While this, of course, provides a significant speedup compared to a sequential computation,
  this approach is not as efficient as one would desire: While most of the entries require only less
  then $3$ hours to finish, there are also various IBP coefficients
  which decompose in about $72$ hours and thus dominate the overall run-time.

Therefore, we use a second layer of parallelism as described in Sections \ref{sec:parallel} and \ref{Petrinet} to speed up the decomposition of the individual
difficult IBP coefficients. %The most complicated coefficient can then be simplified within $19$ hours on
%$16$ cores using multi-process computing in \textsc{Singular}. A realilzation of this layer of parallelism
%via  a Petri net can still improve the efficiency here significantly, since it
%allows to spread out the handling of individual entries beyond a single node of
%the cluster, and thus ressources can be utilized far more efficiently due to
%better load balancing (the parallel tasks generated by a single entry again are
%not equally difficult). A corresponding implementation will soon be available.
This approach approach was applied to the $5$\% of matrix entries with the largest
filesize, while the rest of the entries were computed in parallel using a simple
serial implementation of PFD. This allowed the full reduction to be performed in
$21$ hours and $25$
minutes on a cluster of $10$ nodes with $52$ cores each. The total CPU time was just
over $332$ days, with the average computation needing about $1$ hour $34$ minutes of
CPU time.
%(standard deviation $6$h$40$m).%
%However, the standard deviation was quite large at $6$ hours $40$ minutes.
The most time consuming entry required $4$ days and $10$ hours of CPU time.
%\todo{add estimate of time spent on each step, and within the steps, what the
%ratio between compute and merge was}

Table \ref{compression table} shows the size of UT basis coefficients
before and after running our multivariate partial fraction algorithm,
and the compression ratio of Feynman integrals with different
numerator degrees respectively.

\begin{table}[ht]
\label{compression table}
\centering
\label{tab-marks}
\begin{tabular}{|c|c|c|c|c}
\hline degree & original size & compressed size & compression ratio\\
\hline 2 & 73.1KB & 52.4KB & 1.4\\
\hline 3 & 23.6MB & 1.69MB & 14\\
\hline 4 & 1.19GB & 20.7MB & 59\\
\hline 5 & 18.4GB & 163MB & 115\\
\hline total & 19.6GB & 186MB & 108\\
\hline
\end{tabular}
\caption{Compression ratio of UT basis IBP reduction coefficients of
  the ``double-pentagon'' integral with different numerator degrees}
\end{table}

The compression ratio trend is shown in Figure \ref{compression
  graph}, and clearly we see that the compression ratio for IBP
reduction coefficients increases with
the complexity of the target integrals.
\begin{figure}[H]
\label{compression graph}
\centering
\includegraphics[width=0.8\textwidth]{compression_ratio.eps}
\caption{Graphic representation of the compression ratio of UT basis IBP reduction coefficients of
  the ``double-pentagon'' integral with different numerator degrees}
\end{figure}


==> module_intersection.tex <==
\subsection{Syzygy equation and module intersection}
In this section, we will introduce the module intersection method for generating IBP relations. 
It originated from the syzygy IBP reduction
method \cite{Gluza:2010ws,Schabinger:2011dz}.

For a given integral to be reduced, the number of IBP relations generated by the module intersection method is much smaller than that for the traditional Laporta algorithm, thus saving lots of computational resources.

The module intersection method is based on the Baikov representation \cite{Baikov:1996cd,Baikov:1996rk},
where an integral is written as
\begin{equation}
I[\alpha_1\dots\alpha_n]=C_E^LU^{\frac{E-D+1}{2}}\int_\Omega {\rm d}z_1\cdots{\rm d}z_nP(z)^{\frac{D-L-E-1}{2}}\frac{1}{{z_1}^{\alpha_1}\cdots{z_n}^{\alpha_n}},
\end{equation}
where $C_E^L$ is a constant, $U$ is the Gram determinant
\begin{equation}
U={\rm det}G
\begin{pmatrix}
&p_1,&\dots&p_E\\
&p_1,&\dots&p_E
\end{pmatrix},
\end{equation}
$L$ is loop order, $E$ is number of independent external vectors, $P(z)$ is the Baikov polynomial depending on $z={z_i}$, that is,
\begin{equation}
P={\rm det}G
\begin{pmatrix}
l_1,&\dots&l_L,&p_1,&\dots&p_E\\
l_1,&\dots&l_L,&p_1,&\dots&p_E
\end{pmatrix},
\end{equation}
which vanishes on the boundary $\partial \Omega$.

In Baikov representation, the IBP relations come from
\begin{equation}\label{eq:Baikov IBP}
0=\int_\Omega {\rm d}z_1\cdots{\rm d}z_n\sum_{i=1}^{n}\frac{\partial}{\partial z_i}\Big(a_i(z)P(z)^{\frac{D-L-E-1}{2}}\frac{1}{{z_1}^{\alpha_1}\cdots{z_n}^{\alpha_n}}\Big),
\end{equation}
where $a_i$'s are some polynomials that depend on $z={z_i}$'s. The expansion of equation \eqref{eq:Baikov IBP} gives an IBP relation, if the chosen $a_i(z)$'s satisfy such condition that there exists some polynomial $b(z)$ that
\begin{equation}\label{eq:Baikov syzygy}
\Big(\sum_{i=1}^na_i(z)\frac{\partial P}{\partial z_i}\Big)+b(z)P=0.
\end{equation}
Equation \eqref{eq:Baikov syzygy} is called a syzygy equation for generators $\{P,\frac{\partial P}{\partial z_1},\dots,\frac{\partial P}{\partial z_n}\}$, where the $a_i(z)$'s and $b(z)$ form a solution for this syzygy equation, and each solution corresponds to an IBP relation. Note that traditional methods have no control on the power increase while generating IBP relations, which we want to prevent for simplicity of the calculation. The syzygy method can nicely control the power of index while generating IBP relations, preventing them from increasing by adding an additional constraint
\begin{equation}\label{eq:power control syzygy}
a_i(z)=z_ib_i(z),\quad i\in\mathcal{S},
\end{equation}
where $b_i(z)$'s are polynomials in $z_i$'s and $\mathcal{S}$ is the set of indices of which the power needs to be prevented from increasing.

Solving equation \eqref{eq:Baikov syzygy} is not a computationally hard task.  See the ref.~\cite{Ita:2015tya} for resolving this constraint by the canonical form of IBP relations. Here we use a Laplacian expansion to solve this constraint~\cite{Boehm:2017wjc}.  Since the Baikov polynomial is a determinant, that is, $P=\det(P_{ij})$, we have a Laplace expansion as
\begin{equation}\label{eq:Laplace expansion of determinant}
\sum_jP_{kj}\frac{\partial P}{\partial P_{ij}}-\delta_{ki}P=0.
\end{equation}
The derivative with respect to matrix entries $\frac{\partial P}{\partial P_{ij}}$ can  easily be converted to a derivative with respect to $z_i$'s, that is $\frac{\partial P}{\partial z_i}$, via the Leibniz chain rule. Then \eqref{eq:Laplace expansion of determinant} gives the solutions to the syzygy equation \eqref{eq:Baikov syzygy} in form of a module $M_1$, whose generators are at most linear in the $z_i$'s.

The solutions of \eqref{eq:power control syzygy} form another module whose generators are simply $a_i=z_i$, $b_i=1$ for $i\in \mathcal{S}$. The final solution for the equations are then given by the module $M_1\cap M_2$. The module intersection can be performed by a module Gr${\rm \ddot{o}}$bner basis computation in a position-over-term ordering \cite{Boehm:2018fpv}. While calculating the module intersection, we can treat the kinetic variables $c_i$ and the Baikov variables $z_i$ in the same way, that is, we  calculate a Gr${\rm \ddot{o}}$bner basis in the polynomial ring $\mathbb{Q}[c_1,\dots,c_m,z_1,\dots,z_n]$. This will make the calculation faster than taking $c_i$'s as parameters (rather than variables), though resulting in a redundant generating system. Such a redundant result can be imported back to $\mathbb{Q}(c_1,\dots,c_m)[z_1,\dots,z_n]$. By checking the leading term, redundant generators can be removed. This can be done by using the \texttt{simplify} command in \textsc{Singular}. 

Once we have solutions for \eqref{eq:Baikov syzygy} and \eqref{eq:power control syzygy}, we can use \eqref{eq:Baikov IBP} to generate IBP relations whose powers for the specified indices never increase. Such an IBP system is of much smaller numbers of IBP relations and, hence, total size. Usually, we will generate IBP relations on spanning cuts and then assemble the full IBP system, instead of generating the whole system directly. For more details, see \cite{Boehm:2018fpv,Bendle:2019csk}. In this paper, we use our package \textsc{ModuleIntersection} \cite{Bendle:2020iim} to automize the module intersection and the corresponding IBP generation. 

\subsection{Linear reduction of the IBP system}
Once we have obtained the IBP system, we reduce it by using our own algorithm and implementation for linear reduction (\cite{Bendle:2019csk}). First, we find independent IBP relations by perform the reduction  setting the variables to integers and using linear algebra over finite fields. Then, we simplify the linear system via removing the overlap between two different cuts. Then, we use the linear system simplified by the previous steps to reduce the target integrals to master integrals, giving the IBP reduction coefficients as a final result. Note that, in the third step, we rely our own RREF code, which applies not only row but also column swaps, for finding the best pivots. The column operation changes the set of master integrals, but we can convert the new master integrals to the original ones a posteriori. We have observed that adding such column operation makes our calculation much faster.

For some complicated IBP reduction computations, an analytical calculation takes too much time to be doable. Hence, we perform calculations semi-numerically in such cases. This is to set some but usually not all variables to some constant integers and then perform the reduction. This results in a much lower cost for the computation. %In practice, we can treat one of the variables (including $c_i$'s and spacetime dimension parameter $\epsilon$) as an analytic variable and set the remaining ones to constant integers. 
After the reduction, from the semi-analytic result we can determine the degree of the chosen-analytic variable in each IBP coefficient (usually a rational function). Knowing the degree for each variable, we can perform reduction on multiple semi-numeric points, to interpolate the fully analytic IBP coefficients. The rational function interpolation algorithm is described in Appendix A of ref.~\cite{Bendle:2019csk}. However, observations in ref.~\cite{Boehm:2020ijp} can help us to convert the problem from rational function interpolation to polynomial interpolation, with the latter one being easier. 

To be specific, as observed in ref.~\cite{Boehm:2020ijp}, the denominator factors of IBP coefficients only contain symbol letters or simple polynomials in $\epsilon$, if a UT basis is chosen as the master integrals. (See ~\cite{Henn:2013pwa,Henn:2014qga} for an overview of UT integrals. See ~\cite{Goncharov:2010jf,Duhr:2011zq,Duhr:2012fh} for an overview of symbols.) With this knowledge, for determination of orders for factors in $\epsilon$, we carry out a reduction by setting all kinetic variables as constants and leave $\epsilon$ analytic. For determination of power for symbol letters in the denominators, we set $\epsilon$ as a constant and kinetic variables as generically arbitrary linear functions in an auxiliary variable $x$, such that all symbol letters are distinct in this parameterization.  Then we carry out a reduction, and the orders for symbol letters in the denominators can be read by factorizing the denominator expressions in $x$.

After getting the analytic result for the denominators, we then need to interpolate the numerators via polynomial interpolation. The degree of each variable in the numerators can be acquired by performing the reduction after setting all but one variable as constant integers, as previously stated. Once the degree of variables is known, interpolation of corresponding polynomial becomes a well-defined problem. One needs to accumulate $\prod(d_i+1)$ semi-numeric points, where $d_i$ is the degree for the $i$-th variable to be interpolated, and then carry out reduction on these points. The analytic expressions for these numerators can be interpolated from these semi-numeric results. 

There is another point for simplifying the calculation which we will mention here: Since IBP coefficients are homogeneous in the kinetic variables, we can set one of them, e.g., $c_1$, to 1, and do the steps stated above, determining the analytic result of IBP coefficients with $c_1=1$. Then we can restore the final result with $c_1$ dependence via dimension analysis. %This will make the computation easier than directly interpolating the analytic result with $c_1$ dependence.






